GridToPix: Training Embodied Agents with Minimal Supervision

While deep reinforcement learning (RL) promises freedom from hand-labeled data, great successes, especially for Embodied AI, require significant work to create supervision via carefully shaped rewards. Indeed, without shaped rewards, i.e., with only terminal rewards, present-day Embodied AI results degrade significantly across Embodied AI problems from single-agent Habitat-based PointGoal Navigation (SPL drops from 55 to 0) and two-agent AI2-THOR-based Furniture Moving (success drops from 58% to 1%) to three-agent Google Football-based 3 vs. 1 with Keeper (game score drops from 0.6 to 0.1). As training from shaped rewards doesn't scale to more realistic tasks, the community needs to improve the success of training with terminal rewards. For this we propose GridToPix: 1) train agents with terminal rewards in gridworlds that generically mirror Embodied AI environments, i.e., they are independent of the task; 2) distill the learned policy into agents that reside in complex visual worlds. Despite learning from only terminal rewards with identical models and RL algorithms, GridToPix significantly improves results across tasks: from PointGoal Navigation (SPL improves from 0 to 64) and Furniture Moving (success improves from 1% to 25%) to football gameplay (game score improves from 0.1 to 0.6). GridToPix even helps to improve the results of shaped reward training.

==> ICCV21 Grid to Pixels (1)_arXiv/sections/00_abstract.tex <==
\begin{abstract}
While deep reinforcement learning (RL) promises freedom from  hand-labeled data,   great successes, especially for  Embodied AI, require significant work to create supervision via carefully shaped rewards.
Indeed, without shaped rewards, \ie, with only  terminal rewards, present-day Embodied AI results degrade significantly across Embodied AI problems from single-agent Habitat-based PointGoal Navigation (SPL drops from 55 to 0) and two-agent AI2-THOR-based Furniture Moving (success drops from 58\% to 1\%) to three-agent Google Football-based \footballtask (game score drops from 0.6 to 0.1). 
As training from shaped rewards doesn't scale to more realistic tasks, the community needs to improve the success of training with terminal rewards.  
For this we propose \gtop: 1) train agents with terminal rewards in gridworlds that generically mirror Embodied AI environments, \ie, they are independent of the task; 2) distill the learned policy into agents that reside in complex visual worlds. Despite learning from only terminal rewards with identical models and RL algorithms, \gtop significantly improves results across  tasks: from PointGoal Navigation (SPL improves from 0 to 64) and Furniture Moving (success improves from 1\% to 25\%) to football gameplay (game score improves from 0.1 to 0.6). \gtop even helps to improve the results of shaped reward training. %
\iffalse
While deep reinforcement learning (RL) promises freedom from having to construct large, hand-labelled datasets, the  great successes of deep RL, especially in the Embodied AI domain, have required extensive supervision in another form: carefully shaped rewards.
In this work, we show that in the absence of human supervision and shaped rewards, present-day methods degrade significantly across a suite of Embodied AI problems. To rectify this, we propose \gtop\ -- an approach that first trains agents in mirrored gridworld environments with terminal rewards and then distils the learned policies into agents that reside in complex visual worlds. The proposed gridworlds are easy to generate and need to be designed only once to mirror a visual environment. Once designed they are  applicable across tasks. Importantly, we find that this distillation enables the learning of high-quality policies within visual environments without the extensive, time consuming, reward shaping commonly required. These results move us closer to the grand goal of enabling embodied agents to learn with minimal or no human intervention.
\fi



\end{abstract}

==> ICCV21 Grid to Pixels (1)_arXiv/sections/01_introduction.tex <==
\vspace{-2mm}
\section{Introduction} \label{sec:intro}
\begin{figure}[t]
    \centering
    \includegraphics[trim=10 5 10 3,clip,width=\linewidth]{figs/iccv_teaser_v9.pdf}
    \vspace{-2mm}
    \caption{\textbf{Shaped \vs terminal rewards.} Across three tasks, embodied AI agents fail to learn from terminal rewards using standard RL methods despite achieving high performance when given carefully shaped rewards. When using our \gtop methodology, the embodied AI agents successfully learn from terminal rewards and  sometimes even outperform DirectPix trained agents receiving shaped rewards.}
    \vspace{-2mm}
    \label{fig:teaserNew}
\end{figure}

\begin{figure*}
    \centering
    \vspace{-1mm}
    \includegraphics[width=0.9\textwidth]{figs/teaser-overview-v4.pdf}
    \vspace{-1mm}
    \caption{\textbf{\gtop methodology to transfer knowledge from gridworld to visual agents.}
    We propose to train agents in gridworld environments, where perception is simplified and simulation is fast, mirroring visual environments used in Embodied AI research. Learned gridworld policies can then be distilled to visual agents via imitation learning. See~\secref{sec:super-vis-agents-via-grid} for detailed notation.}\label{fig:teaser}
\end{figure*}
The Embodied AI research community has developed a host of capable simulated environments focused on the challenges of navigation~\cite{habitat19iccv,xia2018gibson}, interaction~\cite{ai2thor,igibson,Gan2020ThreeDWorldAP}, manipulation~\cite{SAPIEN,RLBench,MetaWorld}, and simulation-to-real transfer~\cite{robothor,pyrobot2019,Sim2RealHabitat}. Fast progress has been made within these environments over the past few years, particularly in navigation heavy tasks such as PointGoal navigation~\cite{habitat19iccv,wijmans2019dd}.

While early applications of deep RL to Embodied AI set down the more challenging path of learning from terminal rewards\footnote{\Ie, reward structures in which the only \emph{goal dependent reward} is given at the end of an episode. Goal independent rewards, \eg, a time-step penalty, can be given at every step.}~\cite{ZhuARXIV2016}, the pursuit of increasingly capable agents has steered us towards employing large amounts of human supervision~\cite{shridhar2020alfred,anderson2018vision,thomason2020vision,hahn2020you,ku2020room}, reward shaping~\cite{wijmans2019dd,wang2019reinforced}, and task-specific architectures~\cite{Chaplot2020Explore,ramakrishnan2020occant}. %
The multitude of rewards and auxiliary hyperparameters that are manually tuned when training Embodied AI agents today is reminiscent of %
careful feature engineering~\cite{sift,hog,Lazebnik2006BeyondBO} in computer vision years ago.

While these design choices have got our field (and agents) off the ground, it is hard to believe that this methodology will scale as  tasks increase in complexity and physical realism. Instead, we must borrow from the notable successes of reinforcement learning in games~\cite{Silver2017MasteringTG,Silver2018AGR}, where sophisticated agents are  trained with  minimal supervision in the form of terminal rewards.

As a first step towards this goal, we empirically analyze the ability of modern tried-and-true Embodied AI algorithms to learn high-quality policies from only  terminal rewards in visual environments (DirectPix). We consider a variety of challenging tasks in three diverse simulators -- single-agent PointGoal Navigation in Habitat~\cite{habitat19iccv} (SPL drops from 55 to 0), two-agent Furniture Moving in AI2-THOR~\cite{ai2thor} (success drops from 58\% to 1\%), and three-agent \footballtask in the Google Research Football Environment~\cite{GoogleResearchFootball} (game score drops from 0.6 to 0.1). Given only  terminal rewards, we find that performance of these modern methods degrades drastically, as summarized in Fig.~\ref{fig:teaserNew}. Often, no meaningful policy is learned despite training for millions of steps. These results are eye-opening and a reminder that we are still ways off in our pursuit of embodied agents that can %
learn skills with minimal supervision, \ie, supervision in the form of only terminal rewards.

If present-day RL algorithms have been successful in other domains (particularly ones requiring less visual processing~\cite{Silver2017MasteringTG,Silver2018AGR,babyai_iclr19}), why do they struggle for Embodied AI? Our hypothesis: this struggle is due to the need for embodied agents to learn to plan and perceive simultaneously. This introduces a `non-stationarity' into  learning -- the planning module must continuously adapt to changes in perceptual reasoning. While non-stationarity in learning has also been a problem in past challenges conquered by RL methods, Embodied AI tasks exacerbate this problem due to the presence of rich and diverse visual observations, long-horizon planning, a need for collaboration, and a requirement to generalize to  unseen test worlds.

Driven by this hypothesis, we study \gtop, a 
training routine
for embodied agents that decouples the joint goal of planning from visual input into two manageable pieces. Specifically, using general-purpose \textit{gridworld} environments which generically mirror the embodied environments of interest, we first train a gridworld agent for the desired task.
Within a gridworld, an agent has perfect visual capabilities, allowing learning algorithms to focus on long-horizon planning %
given only terminal rewards. Next, this gridworld agent supervises an agent operating \camera{\textit{solely}} on complex visual observations \camera{(no gridworld is needed at test time). 
Importantly, our conceptualization of `gridworld' isn't restricted to a top-down occupancy map. As we detail in \secref{sec:thor-habitat-gridworlds}, gridworlds are perfect-perception environments, \ie, \textit{semantics are explicitly available} to the agent.} 

Across tasks, as summarized in~\figref{fig:teaserNew}, we observe that \gtop significantly outperforms directly comparable\footnote{\Ie, using identical model architectures.} methods when training visual agents using terminal rewards: for PointGoal Navigation the SPL metric improves from 0 to 64; for Furniture Moving success improves from 1\% to 25\%; for \footballtask the game score improves from 0.1 to 0.6.  
Moreover, \gtop %
even improves
benchmarks when trained with carefully shaped rewards. 
This finding is analogous to the progress made by weakly supervised computer vision approaches which inch towards benchmarks set by fully supervised methods.




\iffalse
\unnat{
Research in reinforcement learning (RL) algorithms have enabled AI agents to learn complex behaviors with mere observations from their interacting environment. RL algorithms do not need a human annotator or a rule-based expert to densely supervised the agent at each step of its trajectory. Instead, RL agents are adept at tracing information from delayed and terminal rewards. We use \textit{terminal rewards} to denote formulations where goal-dependent or win-lose rewards are available only at the termination of an episode.\footnote{Goal-independent rewards may be available at other steps.} For example, an agent receiving a $+1$ for termination with success, $-1$ reward for termination with failure, and time-step penalty (or negative slack reward) to encourage speed.

To bring RL closer to real-world applications, perceptually realistic simulators have been designed. This allows agents to operate with visual, aural, and linguistic observations~\cite{}. Subsequently, user-friendly APIs like AIHabitat~\cite{}, AllenAct~\cite{}, Gibson~\cite{}, ...~\cite{} have allowed researchers to easily deploy RL to train perceptual or \textit{embodied agents}. En route to training the initial (visual) embodied agents, in recent years, several design choices were made -- providing dense rewards/supervision being a key one. \tabref{tab:rl-vs-embodied} concretely contrasts the density of supervision adopted in general RL and specifically in embodied AI. 

In this work, we investigate the question: ``how can we train existing agent models for (a diverse sample of) current embodied AI tasks with the minimal supervision of terminal rewards?'' We conduct experiments across three diverse embodied tasks (PointGoal navigation, Furniture Moving, Google Research Football), each based on a different visual simulator. Our first result is a negative one: well-studied baselines in the literature struggle to learn with terminal rewards. This is surprising given the success of RL in non-visual or perfect-perception domains.

Our hypothesis for the above finding is that visual agents must plan and perceive simultaneously (unlike non-visual counterparts in RL). This introduces a non-stationarity into the learning dynamics: the planning module must continuously adapt to changes in perceptual reasoning. To test and overcome this, we propose \gtop, a learning strategy that factorizes visual planning into manageable ones via the creation of general-purpose gridworld environments mirroring the embodied environments of interest. Within a gridworld, an agent has perfect visual capabilities, allowing learning algorithms to focus on long-horizon planning and enabling them to learn using only terminal rewards. This gridworld agent is then used to supervise an agent within the far more complex visual worlds. With \gtop, we achieve XYZ.

This work is directed at evaluating the choice of dense supervision for embodied agents and enabling learning these agents with minimal supervision. Across three tasks, we show our proposed \gtop improves over directly training visual agent using RL, given the same policy network architecture. We choose the fundamental network architectures that are most investigated in the literature of corresponding tasks. This work doesn't claim or aim to outperform state-of-the-art by including novel, task-specific, inductive biases to the policy network architecture (spatial memory representation, hierarchical planning~\etc). While essential to embodied AI research, improving deep learning architectures of the agent is orthogonal to our work and can naturally be combined with our training strategy. We request the reader to note this while reading our work.}
\fi







\iffalse
Deep reinforcement learning algorithms are adept at learning from sparse and delayed rewards. Notable success stories in deep reinforcement learning include systems which succeed at %
games %
like
Chess, Go, Shogi, and the Atari 2600 suite -- systems that  learn \emph{tabula rasa}, with minimal domain knowledge or inductive biases, without human data or supervision and with only terminal rewards. 
These successes have led researchers to employ RL algorithms in domains beyond gameplay, as diverse as protein discovery, robotics, blah1 and blah2.

Building upon this success, a long term goal for the AI community is to develop embodied agents capable of assisting humans at complex tasks, \eg,  %
in factories (building, monitoring, quality control) or in situations harmful to humans (disaster relief, rescue). 
However, developing agents to perform such complex tasks requires significant breakthroughs in visual, aural, and linguistic processing as well as algorithms capable of learning with little to no supervision.

While early works in embodied AI set down the more challenging path of learning from terminal rewards, the pursuit of increasingly capable agents has steered us towards employing large amounts of human supervision (cite Alfred and VLN papers), dense reward shaping (cite navigation), as well as custom architectures which explicitly designed for the goal at hand (cite ANM). While these design choices have got our field (and agents) off the ground, %
it is challenging to believe that these approaches will scale as our tasks increase in complexity and physical realism.

In this work, we first analyze the ability of present-day embodied AI learning methods to learn a variety of tasks like navigation and multi-agent cooperation from just sparse terminal rewards. We find that their performance degrades drastically. 
In fact, at the long horizon task of object rearrangement, learning simply does not get off the ground.
If existing RL algorithms have been successful in other domains with only terminal rewards, why do they struggle at the suite of embodied AI challenges? Embodied AI tasks require models to learn to parse rich (visual) observations while, simultaneously, learning to plan long sequences of interactive actions to complete a given task. Moreover, Embodied AI agents are expected to generalize their learned behaviors to a visually distinct, previously unseen, test environments. Having to learn to plan and perceive simultaneously introduces non-stationary into the learning dynamics: the planning module must continuously adapt to changes in perception. We posit that present-day algorithms are simply too inefficient at handling these challenges at once.

We propose \gtop, an learning strategy that factorizes this challenge into more manageable ones via the creation of general purpose gridworld environments mirroring the embodied environments of interest. Within a gridworld an agent has perfect visual capabilities, allowing learning algorithms to focus on long horizon planning and enabling them to learn more easily using only terminal rewards. This capable gridworld agent is then used to supervise an agent within the far more complex visual worlds.

\textit{Our experiments show that: Talk about better numbers + better generalization + faster learning, etc.}

\textit{Last paragraph: In summary:
1. show that terminal rewards cause drops
2. gridworlds offer huge improvements
3. these grid worlds only need to be created once and can be used all emb-AI tasks incl nav and manipulation}
\fi

\iffalse
\noindent \hrulefill \\

A long term goal of our community is  development of intelligent embodied agents that perceive and autonomously interact with their environment to complete a variety of tasks. Training such agents in the real world continues to be extremely challenging for three primary reasons: 1) the high costs of purchasing and maintaining robots, 2) the sample-complexity of learning algorithms,  and 3) the small amount of available training experiences because of the slow speed at which these robots operate. As a result, a growing number of researchers study training of embodied agents in simulated visual  worlds~\cite{ai2thor,habitat19iccv,SAPIEN,Gan2020ThreeDWorldAP,talbot2020benchbot} to perform tasks like navigation~\cite{robothor,wijmans2019dd,ZhuARXIV2016,Chaplot2020Explore}, instruction following~\cite{GordonCVPR2018,krantz2020beyond,anderson2018vision,shridhar2020alfred}, and adversarial gameplay~\cite{weihs2019artificial}. The common hope: transferring policies trained in simulation to real robots~\cite{robothor,Sim2RealHabitat} is easier than training these policies from scratch in the real world.

The most popular simulators employed by Embodied AI researchers are several orders of magnitude faster than robots interacting in the real world. This permits to train embodied agents with modern deep reinforcement learning (RL) techniques. 
To maintain  training efficiency, reward signals have to be immediately accessible an accurate, \ie, a ground-truth expert agent needs to be available. While this is possible for tasks like navigation, the difficulty of computing the ground-truth expert action often increases with the task complexity and often requires additional information like maps. For instance, in a task where two agents are asked to re-arrange furniture, computation of the ground-truth expert action is not feasible because \as{reason?}.

If a ground-truth expert action is not available we commonly resort to heuristically designed intermediate rewards. However, without great care those heuristic intermediate rewards can lead to agents which don't generalize as well and/or overfit to behavior engrained via intermediate rewards. To circumvent these concerns we wonder: how can training remain reasonably effective if only terminal rewards are available?


To answer this question we %
develop the
approach shown in  Fig.~\ref{fig:teaser}, which we refer to as \gtop. It consists of three steps: (1) \as{manually/semi-automatically?} create a gridworld environment mirroring the embodied environment of interest, (2) train an agent within this gridworld using only terminal rewards, and (3) use a relatively small number of samples to distill the knowledge learned by the gridworld agent into an agent which operates on visual observations.

Thanks to their high simulation speeds and clean observations, gridworld environment policies are able to learn from much more training data in much less time and compute. More importantly, in gridworld environments we can do so using terminal rewards only. %
This transforms the earlier question on learning from terminal rewards to: \emph{can gridworlds which mimic the photorealistic environment serve as a basis for successful policy transfer to photorealistic simulators?}

Our results answer the question affirmatively. In the \habitat~\cite{habitat19iccv} environment, we are able to train a \pnav agent to a Success weighted by Path Length (SPL) score of 0.5 in just over 5 million steps in the visual environment, a  speedup of roughly 7$\times$ over a strong comparable baseline. We also demonstrate the effectiveness of this technique on a multi-agent task of furniture moving in the \thor~\cite{ai2thor} environment, where we obtain a roughly 5$\times$ speedup over comparable baselines. Importantly, within  gridworlds we are able to train  policies using only terminal rewards, \ie, without dense rewards, and are then able to transfer these successfully to visual world agents \as{are dense rewards needed for transfer?}. This is in  contrast to our findings in the visual world, where removing dense rewards fails to produce any effective agents within a reasonable number of steps. This \as{may} open the door to move away from  noisy and heuristic dense reward shaping employed today by practitioners for training of embodied agents, which is particularly important as we move towards more complex and involved tasks where reward shaping is difficult. 

\fi

\iffalse

A long term goal of our community is  development of intelligent embodied agents that perceive and autonomously interact with their environment to complete a variety of tasks. Training such agents in the real world continues to be extremely challenging for three primary reasons: 1) the high costs of purchasing and maintaining robots, 2) the sample-complexity of learning algorithms,  and 3) the small amount of available training experiences because of the slow speed at which these robots operate. As a result, a growing number of researchers study training of embodied agents in simulated  worlds~\cite{ai2thor,habitat19iccv,SAPIEN,Gan2020ThreeDWorldAP,talbot2020benchbot} to perform tasks like navigation~\cite{robothor,wijmans2019dd,ZhuARXIV2016,Chaplot2020Explore}, instruction following~\cite{GordonCVPR2018,krantz2020beyond,anderson2018vision,shridhar2020alfred}, and adversarial gameplay~\cite{weihs2019artificial}. The common hope: transferring policies trained in simulation to real robots~\cite{robothor,Sim2RealHabitat} is easier than training these policies from scratch in the real world.

The most popular simulators employed by Embodied AI researchers are several orders of magnitude faster than robots interacting in the real world. This permits to train embodied agents with modern deep reinforcement learning (RL) techniques. Nonetheless, it is quite common in the literature to see training times approach several months of GPU time. For instance, a recent method achieved near perfect Point Navigation in \habitat using 2.5 billion frames of experience and 6 months of GPU time~\cite{wijmans2019dd}. While this is a very impressive feat, note that this method employs perfect RGB-D and location sensors, assumes no actuation noise, and only requires the agent to navigate in a scene, which is a critical sub-goal of task completion but not always the goal itself. Moving to harder tasks and employing noisy sensors and actuators will likely require even more computation. This is very expensive, scales poorly as we wish to train agents on multiple tasks in multiple environments, and importantly places this research firmly beyond all but a few well-established research labs. 

Ironically, simulation hence faces the same problem that  real-world robot training struggles with %
-- training is too slow and expensive. We need something even faster. Since simulation was able to speed things up the first time around, %
why not employ the same strategy again? \emph{Why not build a fast simulator for our not-so-fast simulators?}

A large body of work in deep reinforcement learning employs gridworlds to develop and study new algorithms. Within those gridworlds, agents are largely unburdened by the need to learn to perceive and thereby often learn surprisingly sophisticated policies (\eg, AlphaGo~\cite{SilverNature2016}, Dota 2~\cite{dota2}, Hide \& Seek~\cite{Baker2019EmergentTU}). Moreover, thanks to their high simulation speeds and clean observations, gridworld environment policies are able to learn from much more training data in much less time and compute. %
This raises an important question: \emph{can gridworlds which mimic the photorealistic environment serve as a basis for successful policy transfer to photorealistic simulators?}

To answer this question we %
develop the
approach shown in  Fig.~\ref{fig:teaser}, which we refer to as \gtop. It consists of three steps: (1) \as{manually/semi-automatically?} create a gridworld environment mirroring the embodied environment of interest, (2) train an agent within this gridworld, and (3) use a relatively small number of samples to distill the knowledge learned by the gridworld agent into an agent which operates on visual observations.

Our results answer the question affirmatively. In the \habitat~\cite{habitat19iccv} environment, we are able to train a \pnav agent to a Success weighted by Path Length (SPL) score of 0.5 in just over 5 million steps in the visual environment, a  speedup of roughly 7$\times$ over a strong comparable baseline. We also demonstrate the effectiveness of this technique on a multi-agent task of furniture moving in the \thor~\cite{ai2thor} environment, where we obtain a roughly 5$\times$ speedup over comparable baselines. Importantly, within  gridworlds we are able to train  policies using only terminal rewards, \ie, without dense rewards, and are then able to transfer these successfully to visual world agents \as{are dense rewards needed for transfer?}. This is in  contrast to our findings in the visual world, where removing dense rewards fails to produce any effective agents within a reasonable number of steps. This \as{may} open the door to move away from  noisy and heuristic dense reward shaping employed today by practitioners for training of embodied agents, which is particularly important as we move towards more complex and involved tasks where reward shaping is difficult. 
\fi
















==> ICCV21 Grid to Pixels (1)_arXiv/sections/02_related.tex <==
\section{Related Work}
\label{sec:rel}
\noindent\textbf{Embodied task completion.} Development of visually realistic simulators~\cite{Chang3DV2017Matterport,ai2thor,stanford2d3d,igibson,habitat19iccv} has led to tremendous progress for embodied
agents. Agents are trained for a variety of tasks including multiple variants of indoor navigation~\cite{robothor,habitat19iccv,igibson,AllenAct,zeng2021pushing,weihs2021visual,szot2021habitat}, question answering~\cite{DasCVPR2018,GordonCVPR2018,Wijmans2019EQAPhoto}, instruction following~\cite{anderson2018vision,fried2018speaker,wang2019reinforced,krantz2020beyond,ku2020room,singh2020moca}, adversarial gameplay~\cite{weihs2021learning,chen2020visual}, and multi-agent collaboration~\cite{jain2019CVPRTBONE,JainWeihs2020CordialSync,GoogleResearchFootball,liu2021cooperative,patel2021comon}. 
In this work we have focused on three diverse  tasks, particularly, PointNav~\cite{habitat19iccv}, {\fmove}~\cite{JainWeihs2020CordialSync}, and \footballtask~\cite{GoogleResearchFootball}. In contrast to past works that generally aim to maximize success rates at these tasks using any and all possible supervision, we focus on achieving high performance while using only terminal rewards.

\noindent\textbf{Sparse rewards.} Learning from sparse rewards has long been of interest within the RL community where research has, in large part, focused on visually simple environments. A number of approaches have been proposed: curiosity as intrinsic motivation for exploring diverse states~\cite{pathakICMl17curiosity}, using hindsight to reinterpret ``failed'' trajectories~\cite{AndrychowiczEtAl2017HindsightHER}, curriculum learning~\cite{Bengio2009,FlorensaEtAl2017}, self-play~\cite{Silver2017MasteringTG,Baker2019EmergentTU}, and learning to shape rewards~\cite{Trott2019KeepingYD,Nair2018VisualRL,Ghosh2019LearningAR}. Unlike these approaches, we are interested in enabling models to learn from terminal rewards in visually complex environments. Our \gtop method can be further enhanced by incorporating any of the above ideas: rather than using standard RL to train our gridworld experts we could instead use one of the above methods and, potentially, obtain even better results. As our gridworld experts already learn high quality policies without these methods we leave this for future work.


\noindent\textbf{Accelerating visual reinforcement learning.} Several methods have been proposed to improve the sample and wall-clock efficiency of RL in embodied tasks. For sample efficiency, agents are often optimized with additional auxiliary self-supervised tasks~\cite{zhu2020vision,ye2020auxiliary}. 
For faster training, advances for distributed and decentralized scaling of PPO have been proposed~\cite{wijmans2019dd,LiuNEURIPS2020}. Pertinent to our work, Jain~\etal~\cite{JainWeihs2020CordialSync} developed an \thor-aligned gridworld ($16\times$ faster than \thor~\cite{ai2thor}) to prototype their experiments and scale their tasks to a larger number of agents.

\noindent\textbf{Imitation learning.}
An alternative to reward-based training of agents is imitation of a supervisory policy or demonstrations via behavior cloning~\cite{sammut1992learning,bain1995framework}. \Eg, Data Aggregation (DAgger)~\cite{ross2010efficient,RossAISTATS2011} mitigates the \textit{covariate-shift} that troubles classical behaviour cloning approaches. 
This has been applied to train visual agents via rule-based shortest path experts~\cite{GuptaCVPR2017,DasECCV2018,jain2019CVPRTBONE,WeihsJain2020Bridging}. 
\camera{
For the task of instruction following~\cite{shridhar2020alfred}, separate neural modules for perception and action have shown to improve policies learned by imitating human-annotated data~\cite{singh2020moca}.
Chen~\etal~\cite{chen2020learning} train gridworld agents to predict waypoints for AI driving.
Their privileged agents are trained by
offline behavior cloning of human-labeled trajectories (with
data augmentation). 
Obtaining human-labeled data for dense supervision for sequence prediction can quickly become costly and time-consuming. In contrast, we train visual agents using self-supervised labels from their gridworld counterparts. Since these experts learn by interacting in the gridworld via \textit{minimal supervision} of terminal rewards, no human-labeled data is needed.
}




==> ICCV21 Grid to Pixels (1)_arXiv/sections/04_GridToPix.tex <==

\section{Why Learn From Terminal Rewards?}
Human supervision, hand-written and rule-based expert teachers, shaped rewards, and custom architectures are common when developing increasingly capable embodied agents. Several questions naturally arise when developing %
agents with only minimal supervision.

\noindent\textit{As rule-based optimal experts are frequently available in today's simulated environments and tasks, why not use them for dense supervision at every step?} Admittedly, many present-day embodied tasks are navigational %
which permits computing optimal actions easily using shortest path algorithms. The community is, however, quickly moving to more intricate and physics-based tasks, where rule-based experts are %
computationally expensive or infeasible.
Consider, for example, the games of Go, Hanabi, and Football, or the real world tasks of elderly assistance and disaster relief. It is extremely difficult to devise a heuristic expert, let alone an optimal one, for any of those examples. Creating heuristic experts in these settings is just as, if not more, labor intensive as the reward shaping we hoped to avoid. With these long term pursuits in mind, we think it is important  to study and develop methods that  learn with minimal supervision, including in tasks that are popular today. In this work, optimal actions can be easily computed for the popular Point Navigation task~\cite{habitat19iccv}. But for the other two tasks we consider -- \fmove~\cite{JainWeihs2020CordialSync} and \footballtask~\cite{GoogleResearchFootball} -- no experts are available in the literature and creating such an expert appears to be extremely difficult.

\noindent\textit{If not rule-based experts, how about collecting human annotations?} Deep models need the equivalent of years of expert supervision even for perfect-perception tasks~\cite{babyai_iclr19}.\footnote{BabyAI gridworld~\cite{babyai_iclr19} studies show that ${\sim} 21$M expert actions are needed to train an agent to complete an instruction following task with high-performance. If humans  produce 1 action per second,  246 days of labeling are required.} Embodied AI would undoubtedly require a similar (if not much larger) number of annotations. Collecting these human annotations is labor intensive and must be done for every new task and behavior we wish our agent to complete. This is extremely expensive and intractable for more complex behaviors. In contrast, terminal rewards are easy to provide and allow  years of simulated self-play (tractable in wall-clock time). This goal aligns closely with the pursuits of the AI community -- pre-training with self-supervision and then learning new skills with minimal human help.

\noindent\textit{Why should we expect that computing terminal rewards is easier than computing shaped rewards?} While we can't ``prove'' that terminal rewards are easier to compute than shaped rewards, we believe there is good evidence that this is, in general, the case. Shaped rewards are frequently designed so that they provide, at every step, feedback to the agent about its progress towards achieving the goal. Computing such rewards thus requires  to approximate a `distance,' in terms of agent actions, between an arbitrary state and the goal. It is not hard to construct tasks where computing such a distance is NP-complete (exponential-time with known algorithms). 
In comparison, verifying that an agent has reached a goal (and thus deserves its terminal reward) requires no such search, making it, in principle, an easier problem.\footnote{The entire class of NP-complete problems is one in which verifying solutions is easy (polynomial time) but in which finding these solutions is fundamentally harder (unless P$=$NP).}



\section{\gtop}
\label{sec:app}
We are interested in learning from only terminal rewards a high-performance policy $\mv$ which acts on realistic (\eg, visual) observations within an Embodied AI environment, hereafter called the visual environment. %
However, empirically and irrespective of the task and environment, we find joint learning of perception and planning from terminal rewards (DirectPix) to be extremely challenging, as summarized in Fig.~\ref{fig:teaserNew}.

In contrast, due to their perceptual simplicity, gridworlds are generally extremely fast to simulate, and learning is sample efficient as a gridworld policy $\mg$ needs to devote little effort to learn accurate perception. %
This enables  gridworld agents to rapidly learn high-quality policies $\mg$ from only terminal rewards. 


This advantage of gridworlds is an opportunity to reduce labor-intensive reward shaping efforts: can we first learn policies from terminal rewards within gridworlds that replicate the dynamics of a visual environment and then efficiently transfer these policies to visual agents?

We refer to the approach which is designed to enable this transfer and which is sketched in Fig.~\ref{fig:teaser} as \gtop, and discuss it next. 
In particular, Sec.~\ref{sec:terminal-vs-shaped-rewards}  formalizes terminal and shaped rewards, Sec.~\ref{sec:thor-habitat-gridworlds} describes how we design gridworlds that replicate a visual environment's dynamics, and Sec.~\ref{sec:super-vis-agents-via-grid} details both how we train gridworld agents and how imitation learning can be used to transfer gridworld policies to visual agents.


\subsection{Terminal \vs Shaped Reward Structures}\label{sec:terminal-vs-shaped-rewards}
The reward structure used during training has a substantial impact on  sample efficiency, stability, and quality of the learned policy. Most prior work for the tasks considered in this paper used a shaped reward structure, \ie, the reward obtained by the agent at timestep $t$ can be decomposed into
\begin{align}
    r^{\text{shaped}}_t =
     r^{\text{success}}_t + r^{\text{progress}}_t + r^{\indep}_t \quad. \label{eq:rewards_dense}
\end{align}
Here, $r^{\text{success}}_t$ is a sparse terminal reward equalling 0 on all but the last timestep; for our considered tasks,
\begin{align}
    \hspace{-0.2cm} r^{\text{success}}_t \!\!=\!  \begin{cases}
     \!r_{\text{success}}\cdot(1 \!-\! \alpha\cdot \frac{t}{T}) & \hspace{-0.3cm}\text{if goal achieved,}\\
     \!0 & \hspace{-0.3cm}\text{otherwise,}
    \end{cases}\label{eq:rewards_terminal}
\end{align}
where $T\geq 1$ is the maximum allowed episode length and $r_{\text{success}}> 0$, $\alpha\in[0,1]$ are task-specific constants.\footnote{The inclusion of the $\alpha$ parameter in terminal rewards allows to encode a more nuanced measure of success. Note that when  $\alpha>0$, $r^{\text{success}}_t$ is larger when the agent completes the task in fewer steps.}
Further, $r^{\text{progress}}_t$ is a dense, goal-dependent reward, often equalling the change in distance to the goal. %
Finally, $r^{\indep}_t$ is a possibly dense but goal-independent reward, meant to encourage behaviors that are generally thought to be ``good'' regardless of the task, \eg, $r^{\indep}_t$ often includes a small negative step penalty which gently encourages the agent to complete its task quickly. 

As previously discussed, the goal-dependent shaped rewards $r^{\text{progress}}_t$ must be manually designed, can be computationally expensive, and generally require privileged access to the environment state. Because of this, we often aim to train  agents with the simpler reward structure
\begin{align}
    r^{\text{terminal}}_t =
     r^{\text{success}}_t + r^{\indep}_t \quad. \label{eq:rewards_simple}
\end{align}
In fact, for our experiments with terminal rewards, we let $r^{\indep}_t \equiv 0$  in all but the \fmove task where we keep prior work's inclusion of a step and failed-coordination penalty.





\subsection{Gridworld Mirrors of Visual Environments}
\label{sec:thor-habitat-gridworlds}

In order for policies obtained from gridworld training to be successfully transferable to visual agents, we need these gridworlds to be mirrors of their visual counterparts: a step in the gridworld should be translatable to a step in the visual world. 
We will now describe the three gridworlds used in our experiments, mirroring the \habitat, \thor, and Google Football environments. While these gridworlds work well for the considered tasks, they are also applicable for other tasks trained in these environments. We hope to encourage current and future Embodied AI environment developers to provide comprehensive general purpose gridworlds corresponding to their environments.



\noindent\textbf{\textsc{Grid-Habitat}.} 
We extend the existing functionality of the \habitat platform to permit, for the first time,  training of gridworld agents. Specifically, we generate an egocentric, top-down, observation with the agent positioned at the bottom facing towards the center (see Fig.~\ref{fig:teaser}). This top-down observation contains sensor information about occupancy (\ie, free space and walls) and goal location. This sensor information is sufficient for \pnav and can be easily enriched for other tasks (\eg, by adding semantic channels for ObjectNav). Our gridworld observation is different from the top-down visualization tool provided by \habitat which is allocentric and scaled differently for different scenes. We call this new gridworld \textsc{Grid-Habitat}. 

\noindent\textbf{\textsc{Grid-AI2-THOR}.} For the multi-agent {\fmove} task, we follow Jain~\etal~\cite{JainWeihs2020CordialSync} and conduct our study on an \thor-mirroring top-down gridworld.
Given the complexity of \fmove, we include information in separate channels of the top-down tensor with each channel corresponding to the output of a distinct sensor. These sensors specify whether a cell can be occupied by a furniture item, whether the cell is reachable by an agent, whether it was previously visited, the location of the furniture item, and the location of the other agent. We refer to this gridworld as \textsc{Grid-\thor}.

\noindent\textbf{\textsc{Grid-Google-Football}.} For the multi-agent Google football environment 
created by Kurach~\etal~\cite{GoogleResearchFootball}, we construct an observation that summarizes important game state information. Specifically, 
for each controlled player, the gridworld observation is a 1D vector which contains the location of all other players, the ball, and the opponent goal relative to the controlled player's location.


\camera{Importantly, as suggested in \secref{sec:intro}, our conceptualization of a gridworld goes beyond a spatial top-down occupancy map. While observations of \textsc{Grid-Habitat} capture occupancy and goal information, the observation of \textsc{Grid-AI2-THOR} is a tensor containing \textit{explicit semantics} of the environment. Moreover, as in \textsc{Grid-Google-Football}, gridworld observations need not be restricted to have spatial structure. Here, as is common in RL literature, gridworld agents receive a 1D vector capturing perfect-perception observations.}

\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{figs/model-diagram-v3.pdf}
    \vspace{-1mm}
    \caption{\textbf{Model overview.} Schematic of how top-down grid and visual observations are processed by their respective networks. The gridworld agent is trained via actor-critic losses, and subsequently supervises the visual agent via a cross-entropy loss.
    }
    \label{fig:overview}
\end{figure}


\subsection{Supervising Visual Agents via Gridworlds}\label{sec:super-vis-agents-via-grid}

We now describe how we train  gridworld agents and subsequently use imitation learning to transfer their learned policies to visual agents. An overview is given in Fig.~\ref{fig:overview}.

\noindent\textbf{Training in Gridworlds.}
As is standard in RL, we train gridworld agents to maximize the expected $\gamma$-discounted cumulative reward of their actions. Task specific details (\eg, algorithms and hyperparameters) are included in~\secref{sec:tasks}.
Whenever possible we follow protocols laid out by prior work.

\noindent\textbf{Distilling policies.}
How can we effectively train the parameters of a visual agent policy $\mv$ given a policy $\mg$ trained in a gridworld? 
To answer this question, recall that the visual agent $\av$ is interacting with a visual environment for which every step is translatable to a gridworld. The visual agent can hence be supervised by a gridworld agent $\ag$. 
The visual agent $\av$ might act using its own policy $\mv$ or adopt an \textit{exploration policy} $\mu$. This leads to on-policy and off-policy variants of imitation learning (IL). To illustrate this, let a rollout of the visual agent $\av$ and the  gridworld agent $\ag$  be $(a_1^{\av}, a_2^{\av},  \dots, a_t^{\av})$ and $(a_1^{\ag}, a_2^{\ag}, \dots, a_t^{\ag})$, respectively. To train the parameters of the visual policy $\mv$ via \gtop, we employ  the  cross-entropy loss. Formally, suppose that $O_\mu$ is a random variable corresponding to the observation seen by an agent when following policy $\mu$ and suppose that $H_\mu$ is a random variable encoding the history of all observations seen before obtaining observation $O_\mu$. The \gtop loss is then
\begin{equation}
    \mathcal{L}_{\text{\gtop}} = \mathbb{E}[\mathbb{E}_{a\sim\mg(\cdot \mid O_\mu, H_\mu)}[-\log\mv(a\mid O_\mu, H_\mu)]]. 
\end{equation}
The choice of exploratory policy $\mu$ leads to three variants, each widely adopted in IL %
tasks: %
\camera{ student forcing, teacher forcing, and annealed teacher forcing or DAgger (details in Appendix).}
In our experiments we primarily use DAgger.
Importantly, no matter the exploration policy used during training, at test time the visual agent's policy $\mv$ is deployed so that there is no access to gridworld policies at test time. 






 

==> ICCV21 Grid to Pixels (1)_arXiv/sections/05_experiments.tex <==
\section{Tasks, Models, and Evaluation}
\label{sec:tasks}
We evaluate \gtop using three tasks. We  chose these tasks as they (a) span both single-agent and multi-agent settings, (b) include tasks that do not have easily constructed rule-based experts (\fmove and \footballtask Football) as well as a task for which optimal actions can be computed from shortest path computations (\pnav), (c) provide the opportunity to test \gtop across a variety of different reward structures and model architectures, and (d) employ three different Embodied AI environments. 
\camera{Additionally, in the Appendix, we include experiments for a task where \textit{perfect reward shaping is intractable} -- Visual Predator-Prey (in OpenAI multi-particle environment~\cite{LoweNIPS2017,MordatchAAAI2018}).}
Across all experimental results, we present %
standard evaluation metrics after 10\% and 100\% of training has completed (to provide an understanding of sample efficiency and asymptotic results).

\subsection{PointGoal Navigation}
\label{sec:task-pnav}
PointGoal Navigation (\pnav) is a single agent navigation task specified for the \habitat\ simulator. An agent is spawned at a random location in the scene and must navigate to a target location specified by  coordinates relative to the agent's current location.  The relative goal position is available at every time step and the agent navigates by choosing one of four actions at every step.

\noindent\textbf{Shaped rewards.} Traditionally trained with shaped rewards~\cite{habitat19iccv,wijmans2019dd,ye2020auxiliary}, the change in shortest-geodesic-path distance to the goal is chosen as the goal-dependent progress reward $r^{\text{progress}}_t$ (see~\equref{eq:rewards_dense}). Computing it requires access to the full scene graph and a shortest-path planner. Here the success reward $r^{\text{success}}_t$ is chosen as in Eq.~\eqref{eq:rewards_terminal} with $r_{\text{success}}=10$ and $\alpha=0$. Finally, $r^{\indep}_t$ is a constant step penalty of $-0.01$.

\noindent\textbf{Terminal rewards.} Here we use the reward structure from \equref{eq:rewards_simple} with $r_t^\text{success}$ obtained from 
\equref{eq:rewards_terminal} with $r_{\text{success}}=10$ and $\alpha=0.9$. We set $r_t^{\indep} = 0$.

\noindent\textbf{Model architecture.} For a fair comparison, we use the standard CNN-GRU architecture~\cite{habitat19iccv,wijmans2019dd,chen2019audio,cartillier2020semantic,chang2020semantic,wani2020multion}. We adopt the official  implementation\footnote{github.com/facebookresearch/habitat-lab} and train with PPO~\cite{schulman2017proximal}, the de-facto standard RL algorithm for \pnav.


\noindent\textbf{Evaluation.} \pnav agents are primarily evaluated via Success weighted by Path Length (SPL)~\cite{anderson2018evaluation} and percentage of successful episodes (Success). We set a budget of 50 million environment steps\footnote{${\sim}2.5$ days of training using a \emph{g4dn.12xlarge} AWS instance configured with 4 NVIDIA T4 GPUs, 48 CPUs, and 192 GB memory.} and report results on the Gibson validation set of 14 unseen scenes with 994 episodes.





\begin{table*}[t]
\vspace{-0.2cm}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{l>{\columncolor{ColorPNav}}c>{\columncolor{ColorPNav}}c>{\columncolor{ColorPNav}}c>{\columncolor{ColorPNav}}c>{\columncolor{ColorFurnMove}}c>{\columncolor{ColorFurnMove}}c>{\columncolor{ColorFurnMove}}c>{\columncolor{ColorFurnMove}}c>{\columncolor{ColorFootball}}c>{\columncolor{ColorFootball}}c}

\toprule
\multicolumn{1}{c}{Tasks $\rightarrow$} & \multicolumn{4}{c}{\cellcolor{ColorPNav}\textbf{PointGoal Navigation}} & \multicolumn{4}{c}{\cellcolor{ColorFurnMove}\textbf{Furniture Moving}} & \multicolumn{2}{c}{\cellcolor{ColorFootball}\textbf{3 \vs 1 with Keeper}} \\
\multicolumn{1}{c}{} & \multicolumn{2}{c}{\cellcolor{ColorPNav}SPL} & \multicolumn{2}{c}{\cellcolor{ColorPNav}Success} & \multicolumn{2}{c}{\cellcolor{ColorFurnMove}MD-SPL} & \multicolumn{2}{c}{\cellcolor{ColorFurnMove}Success} & \multicolumn{2}{c}{\cellcolor{ColorFootball}Game Score} \\
Training routines $\downarrow$ & \emph{@10\%} & \emph{@100\%} & \emph{@10\%} & \emph{@100\%} & \emph{@10\%} & \emph{@100\%} & \emph{@10\%} & \emph{@100\%} & \emph{@10\%} & \emph{@100\%} \\
\midrule
\directrl & 0.0 & 0.1 & 0.0 & 0.2 & 0.0 & 0.0 & 0.8 & 0.8 & 0.03 & 0.07 \\
\gtop & \textbf{45.4} & \textbf{63.8} & \textbf{63.5} & \textbf{81.8} & 1.6 & \textbf{4.0} & 16.4 & \textbf{24.6} & 0.33 & \textbf{0.63} \\
\gtop $\rightarrow$ \directrl & 44.6 & 59.7 & 62.1 & 77.7 & \textbf{2.7} & 3.1 & \textbf{19.8} & 14.5 & \textbf{0.35} & 0.6 \\
\midrule
Gridworld expert (\textit{upper bound}) & \multicolumn{2}{c}{\cellcolor{ColorPNav}\textit{78.8}} & \multicolumn{2}{c}{\cellcolor{ColorPNav}\textit{94.2}} & \multicolumn{2}{c}{\cellcolor{ColorFurnMove}\textit{19.2}} & \multicolumn{2}{c}{\cellcolor{ColorFurnMove}\textit{56}} & \multicolumn{2}{c}{\cellcolor{ColorFootball}\textit{0.9}} \\
\bottomrule
\end{tabular}%
}
\vspace{0.03in}
\caption{\textbf{Quantitative results (terminal reward structure).} Metric values for the \pnav, \fmove, and \footballtask tasks reported on their respective evaluation sets (see~\secref{sec:tasks}). Across all the three tasks, the \gtop agents outperform their \Directrl counterparts. For ease of reading, SPL is scaled by 100 and success \% is reported. To quantify the efficiency of learning, metrics are reported after \textit{10\%} and \textit{100\%} of training has completed. The last row is separated to highlight that gridworld experts serve as a loose \textit{upper bound} for \gtop agent performance and should otherwise not be directly compared against.
}
\label{tab:terminal-metrics}
\end{table*}







\begin{figure*}[t]
\vspace{-0.3cm}
    \centering
    \begin{tabular}{ccc}
        \multicolumn{3}{c}{\includegraphics[width=0.7\textwidth]{figs/legend_no_variants.pdf}}\vspace{-2mm}\\
        \includegraphics[trim=5 5 10 10,clip,width=0.3\textwidth]{figs/iccv21_nolegend_6-4_ICCV_NO_VARIANTS_POINTNAV_TERMINAL__SPL_roll6.pdf} &
        \includegraphics[trim=5 5 10 10,clip,width=0.3\textwidth]{figs/iccv21_nolegend_6-4_ICCV_TERMINAL_GRIDTOPIX__spl_manhattan_roll6.pdf} &
        \includegraphics[trim=5 5 10 10,clip,width=0.3\textwidth]{figs/GRF_sparse_no_legned_544.pdf}\\
        (a) PointGoal Navigation & (b) Furniture Moving & (c) Football -- \footballtask
    \end{tabular}
    \vspace{0.03in}
    \caption{\textbf{Learning curves on validation set (terminal reward structure).} Primary metrics are plotted \vs training steps/episodes, following the standard protocols for the respective task (see~\secref{sec:tasks}).
    (a) Thin lines mark checkpoints evenly spaced by $1$ Mn frames. Bold lines and shading mark the rolling mean (with a window size of $2$) and the corresponding standard deviation. (b) In line with~\cite{JainWeihs2020CordialSync}, we log information by running an online validation process and employ a local quadratic regression smoothing with 95\% confidence intervals. (c) The plot shows the average game score and standard deviation. Checkpoints are evenly spaced by $200$K frames.
    Despite considerable effort, \Directrl methods  fail to learn meaningful policies with terminal rewards.
    }
    \label{fig:terminal-plots}
    \vspace{-0.1in}
\end{figure*}

\subsection{Furniture Moving}
\label{sec:task-fmove}
\task is a challenging two-agent furniture moving task set within the \thor\ simulator~\cite{JainWeihs2020CordialSync}. Two agents collaborate to move an object through the scene and place it above a visually distinct target. Agents may communicate with other agents at each timestep using a low bandwidth communication channel. Each agent can choose from 13 actions. Specifically, in addition to the vanilla navigation, agents may move with the lifted object, move just the object, and rotate the object. Moreover, due to two agents, the joint action space contains 169 actions. 

\noindent\textbf{Shaped rewards.} Here, change in Manhattan distance to the goal\footnote{In \fmove, computing the shortest-geodesic-path is intractable as each location of the furniture corresponds to over 400k states~\cite{JainWeihs2020CordialSync}.} is used as the goal-dependent reward $r^{\text{progress}}_t$. Three goal-independent rewards are suggested in~\cite{JainWeihs2020CordialSync} to help learn the coordinated policy for this multi-agent system. In particular, $r^{\indep}_t$ includes a step penalty, a joint-pass (or do-nothing) penalty, and a failed action penalty. 

\noindent\textbf{Terminal rewards.} For a head-on comparison with~\cite{JainWeihs2020CordialSync} we simply drop $r^{\text{progress}}_t$. Like prior work~\cite{JainWeihs2020CordialSync}, the success reward $r_t^\text{success}$ is obtained from \equref{eq:rewards_terminal} using  $r_{\text{success}}=1$ and $\alpha=0$.
All \fmove results are based on this. Additional results with $r^{\indep}_t=0.01$ are included in the appendix.

\noindent\textbf{Model architecture.} We utilize SYNC, the best-performing  architecture from prior work~\cite{JainWeihs2020CordialSync}.
For fairness, we use the same RL algorithm (A3C~\cite{MnihEtAlPMLR2016}) as prior work.

\noindent\textbf{Evaluation.} \task agents are primarily evaluated via two metrics -- \% successful episodes (Success) and a Manhattan distance based SPL (MD-SPL). Additional metrics are reported in the appendix. Consistent with~\cite{JainWeihs2020CordialSync}, we train for 500k episodes for the visual agents.\footnote{2-4 days of training with a \emph{g4dn.12xlarge} AWS instance.} Metrics are reported on the test set and learning curves on validation.

\subsection{Football -- \footballtask}
\label{sec:task-football}
\footballtask is a task introduced by Kurach~\etal~\cite{GoogleResearchFootball}. In this multi-agent task, three agents collaborate to score against rule-based defenders.
One agent starts behind the penalty arc and the other two agents start on the sides of the penalty area. There are two opponent rule-based defenders, including one goalkeeper. At the beginning of each episode, the center agent possesses the ball and faces the defender. The episode terminates when the controlled agents score or the maximum episode length is reached. 

\noindent\textbf{Shaped rewards.} We use the `checkpoint'~\cite{GoogleResearchFootball} reward as the goal-dependent reward $r^{\text{progress}}_t$ to encourage  controlled agents to move the ball towards the opponent's goal.
Specifically, the area between the initial location of the center agent and the opponent goal is divided into three checkpoint regions according to the distance to the opponent goal.
A progress reward of $+0.1$ is received the first time the controlled players posses the ball in a checkpoint region.   

\noindent\textbf{Terminal rewards.} Following  \cite{GoogleResearchFootball}, $r_{\text{success}}=1$ and $\alpha=0$.

\noindent\textbf{Model architecture.} For a fair comparison, we use the CNN architecture used by~\cite{GoogleResearchFootball, LiuNEURIPS2020}, and a parallel PPO algorithm~\cite{LiuNEURIPS2020} to train the agents.

\noindent\textbf{Evaluation.} Agents are evaluated using the average score obtained in test episodes. Consistent with Liu~\etal~\cite{LiuNEURIPS2020}, we set a training budget of $8$ million environment steps. Training curves and final metrics are reported on test episodes. 








\begin{table*}[t]
\vspace{-0.2cm}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{l>{\columncolor{ColorPNav}}c>{\columncolor{ColorPNav}}c>{\columncolor{ColorPNav}}c>{\columncolor{ColorPNav}}c>{\columncolor{ColorFurnMove}}c>{\columncolor{ColorFurnMove}}c>{\columncolor{ColorFurnMove}}c>{\columncolor{ColorFurnMove}}c>{\columncolor{ColorFootball}}c>{\columncolor{ColorFootball}}c}

\toprule
\multicolumn{1}{c}{Tasks $\rightarrow$} & \multicolumn{4}{c}{\cellcolor{ColorPNav}\textbf{PointGoal Navigation}} & \multicolumn{4}{c}{\cellcolor{ColorFurnMove}\textbf{Furniture Moving}} & \multicolumn{2}{c}{\cellcolor{ColorFootball}\textbf{3 \vs 1 with Keeper}} \\
\multicolumn{1}{c}{} & \multicolumn{2}{c}{\cellcolor{ColorPNav}SPL} & \multicolumn{2}{c}{\cellcolor{ColorPNav}Success} & \multicolumn{2}{c}{\cellcolor{ColorFurnMove}MD-SPL} & \multicolumn{2}{c}{\cellcolor{ColorFurnMove}Success} & \multicolumn{2}{c}{\cellcolor{ColorFootball}Game Score} \\
Training routines $\downarrow$ & \emph{@10\%} & \emph{@100\%} & \emph{@10\%} & \emph{@100\%} & \emph{@10\%} & \emph{@100\%} & \emph{@10\%} & \emph{@100\%} & \emph{@10\%} & \emph{@100\%} \\
\midrule
\directrl & 35.9 & 54.7 & 60.5 & 79.0 & 2.8 & 11.2 & 22.5 & 58.4 & 0.0 & 0.6 \\
\gtop & \textbf{57.6} & 69.0 & \textbf{77.5} & \textbf{86.4} & \textbf{8.4} & 9.7 & \textbf{57.7} & 62.0 & 0.37 & \textbf{0.65} \\
\gtop $\rightarrow$ \directrl & 53.6 & \textbf{69.1} & 71.9 & 84.9 & 7.1 & \textbf{15.3} & 55.3 & \textbf{68.6} & \textbf{0.38} & 0.61 \\
\midrule
Gridworld expert (\textit{upper bound}) & \multicolumn{2}{c}{\cellcolor{ColorPNav}\textit{85.3}} & \multicolumn{2}{c}{\cellcolor{ColorPNav}\textit{97.5}} & \multicolumn{2}{c}{\cellcolor{ColorFurnMove}\textit{22.2}} & \multicolumn{2}{c}{\cellcolor{ColorFurnMove}\textit{76.3}} & \multicolumn{2}{c}{\cellcolor{ColorFootball}\textit{0.95}} \\
\bottomrule
\end{tabular}%
}
\vspace{0.03in}
\caption{\textbf{Quantitative results (shaped reward structure).} 
Identical to \tabref{tab:terminal-metrics} but all methods have been trained with shaped, rather than terminal, rewards. Even with this denser form of supervision, training routines based on \gtop can improve performance of all the metrics across the three tasks.
}
\label{tab:dense-metrics}
\end{table*}

\begin{figure*}[t]
\vspace{-0.3cm}
    \centering
    \begin{tabular}{ccc}
        \multicolumn{3}{c}{\includegraphics[width=0.7\textwidth]{figs/legend_no_variants.pdf}}\vspace{-2mm}\\
        \includegraphics[trim=5 5 10 10,clip,width=0.3\textwidth]{figs/iccv21_nolegend_6-4_ICCV_NO_VARIANTS_POINTNAV__SPL_roll6.pdf} &
        \includegraphics[trim=5 5 10 10,clip,width=0.3\textwidth]{figs/iccv21_nolegend_6-4_ICCV_DENSE_GRIDTOPIX__spl_manhattan_roll6.pdf} &
        \includegraphics[width=0.3\textwidth]{figs/GRF_dense_no_legend_544.pdf}\\
        (a) PointGoal Navigation & (b) Furniture Moving & (c) Football -- 3 \vs 1 with Keeper
    \end{tabular}
    \vspace{0.03in}
    \caption{\textbf{Learning curves on validation set (shaped reward structure).} Follows~\figref{fig:terminal-plots}. As expected, with this additional supervision the performance gap between \gtop and \Directrl methods narrows but can still be substantial (\eg, in the \pnav task). See~\figref{fig:terminal-plots} for legend and plot details.
    \vspace{-0.5cm}
    }
    \label{fig:dense-plots}
\end{figure*}


\section{Experiments}
\label{sec:results}

We now provide an overview of the training routines employed to train our visual and gridworld agents, followed by results on the three tasks.

\subsection{Training Visual Agents}
\label{sec:training-routines-visual}
\noindent For each task (in both the terminal reward and shaped reward settings), we train visual agents in three ways:\\
\noindent\textbf{\Directrl.} We train visual agents (hence, `Pix') using only reward-based RL losses (\ie, PPO or A3C).\\
\noindent\textbf{GridToPix.} Our proposed routine trains visual agents by imitating a corresponding gridworld expert (that we train). As stated before, the expert is only available at training time and  weights are fixed. 
See  appendix for more details.\\
\noindent\textbf{GridToPix$\rightarrow$\Directrl.} This is a hybrid of the above two routines and follows the common practice of `warm-starting' agent policies with supervised/imitation learning and then fine-tuning with reinforcement learning.\footnote{For example, prior works use IL $\rightarrow$ RL to train agents for visual dialog~\cite{visdial_rl}, embodied question answering~\cite{DasECCV2018}, vision-and-language navigation~\cite{wang2018look,wang2019reinforced,jain2019stay}, and emergent communication~\cite{Lowe2020}.}
Additional details are deferred to the appendix.


\subsection{Training Gridworld Experts} 

For each task, the \textit{gridworld expert} utilizes a training routine identical to \Directrl. Gridworld experts observe semantic top-down tensors or 1D state information, unlike the architectures that learn from raw pixels. Hence, we make minimal edits to the CNN that encodes the observations (see appendix for details). 





As described in~\secref{sec:app}, training in gridworlds is very fast. Moreover, gridworlds can, in principle, be optimized to accelerate the environment transitions. Hence, for gridworld variants of each of the three tasks, we train models to near saturation. Importantly, due to difference in state space, models, and training time, the \textit{gridworld expert} rows in~\tabref{tab:terminal-metrics} and \tabref{tab:dense-metrics} shouldn't be compared to visual analogues. They serve as a loose upper-bound for the performance of the visual agents trained with \gtop.

\subsection{Results}
We report  standard evaluation metrics on three tasks. To study sample efficiency, we also show   learning curves.

\noindent\textbf{Terminal rewards} (see \tabref{tab:terminal-metrics} and \figref{fig:terminal-plots}). With perfect perception, gridworld experts can train to a high performance (\eg, 94\% success in \pnav) and guide the learning of visual agents. In sharp contrast, \directrl doesn't learn a meaningful policy in any of the tasks\footnote{We investigated the learned policy qualitatively in the \pnav task and found that the \directrl agent learns the (locally optimal) policy of executing STOP as its first action. We report best number after training over 15 configurations (20M steps each) by varying the entropy coefficient, number of PPO trainers, and random seeds. For \footballtask, the DirectPix agents shoot straight at the goal and are intercepted by the goal-keeper and sometimes pass to another player who fails to receive.} -- demonstrating present day methods' inability to learn from terminal rewards in these visual worlds. Our \gtop variants perform significantly better. For instance, at \pnav, \gtop obtains a respectable SPL of 0.638, inching towards the 0.788 obtained by the gridworld expert. \gtoptod sometimes produces small gains beyond \gtop. As evidenced by learning curves, \gtop learning is also efficient -- most gains come in the early few million steps (0.45 SPL, \ie, 70\% of the final performance in just 5M steps for \pnav). A similar pattern emerges in other tasks -- \directrl cannot learn  meaningful behaviors from terminal rewards with a 0.8\% success and 0.07 game score in \fmove and \footballtask, respectively. Our training routines achieve the best performance. 

In addition to these improvements in the terminal reward structure, we also investigate the training routines in (the more traditional) setting with shaped rewards.

\noindent\textbf{Shaped rewards} (see \tabref{tab:dense-metrics} and \figref{fig:dense-plots}). As seen in past works, \directrl performs well when provided with shaped rewards. Interestingly, \gtoptod also outperforms \directrl in this reward setting in the first two tasks and performs roughly as well on the third task -- an over 25\% relative gain in SPL (\pnav), an over 35\% relative gain in MD-SPL (\task), and an over 8\% relative gain in game score (Football). The efficiency of learning is also high with \gtoptod reaching 83\% of its final SPL in just 5M steps for the \pnav task. Since \pnav is single-agent navigation, we trained an agent using the optimal shortest-path actions via IL.  \gtop   outperforms this baseline with (very) dense supervision.\footnote{By imitating optimal actions, the visual agent can reach a SPL at (10\%, 100\%) = (0.301, 0.687) and success at (10\%, 100\%) = (35.5, 76.7).} 

These results across three tasks running in three  simulators demonstrate the potential of \gtop  as we move towards training with terminal rewards. In addition \gtop also provides meaningful gains in our current Embodied AI training setups that employ shaped rewards. 



 
 







==> ICCV21 Grid to Pixels (1)_arXiv/sections/06_conclusion.tex <==
\section{Conclusion} \label{sec:conc}
Embodied AI progress is slowed by  labor-intensive work %
to manually tweak model architectures, collect human annotations, and/or shape reward functions. We study how  to reduce this effort significantly: for an embodied environment of interest, create a generic gridworld mirror which is visually parsimonious and fast to simulate. Use of this gridworld mirror for \gtop enables one to avoid many task-specific interventions and allows for learning from only terminal rewards: a critical step for complex tasks within physically realistic  environments where generating shaped rewards quickly becomes infeasible.

\noindent\textbf{Acknowledgements:} This work is supported in part by NSF under Grant \#1718221, 2008387, 2045586, MRI \#1725729, and NIFA award 2020-67021-32799. We thank Anand Bhattad, Angel X.\ Chang, Manolis Savva, Martin Lohmann, and Tanmay Gupta for thoughtful discussions and valuable input.



